Diversity Enhanced Narrative Question Generation for Storybooks

Question generation (QG) from a given context can enhance comprehension, engagement, assessment, and overall efficacy in learning or conversational environments. Despite recent advancements in QG, the challenge of enhancing or measuring the diversity of generated questions often remains unaddressed. In this paper, we introduce a multi-question generation model (mQG), which is capable of generating multiple, diverse, and answerable questions by focusing on context and questions. To validate the answerability of the generated questions, we employ a SQuAD2.0 fine-tuned question answering model, classifying the questions as answerable or not. We train and evaluate mQG on the FairytaleQA dataset, a well-structured QA dataset based on storybooks, with narrative questions. We further apply a zero-shot adaptation on the TellMeWhy and SQuAD1.1 datasets. mQG shows promising results across various evaluation metrics, among strong baselines.

==> sections/03_Method_old.tex <==
\graphicspath{{\subfix{../images/}}}

\begin{figure}[t]
\centering
{\includegraphics[scale=0.45]{images/gen.jpg}}
\caption{Overview of recursive generation.}
\label{fig:mQG-gen}
\end{figure}

In this section, we formalize the multi-question generation task and introduce our mQG. We first formulate our task, then describe the structure of mQG. Finally, we explain how our training works with the newly defined maximum question similarity loss for our task.

 \subsection{Task Formulation}
 \label{sec:task}
 The QG task in this paper aims to generate each question using a given context, question type, and the history of questions generated from the same context with the same question type. Mathematically, given the context $(C)$, question type $(QT)$, history of generated questions $(H_i = (Q_1, Q_2, ..., Q_{i-1}))$, this task can be defined explicitly as generating a question, $\hat{Q}$, where:
\begin{equation}
\hat{Q} = \operatorname{{argmax}_{Q_i}}(Prob(Q_i | QT, C, H_i))
\end{equation}
We use 6 wh-words (what, when, where, which, who, why, how) as question types. To extract wh-words from each question, we apply part-of-speech tagging with Spacy\footnote{\url{https://spacy.io/}} English Model. In a training process, as we do not have a history of generated questions and have an insufficient number of questions per context per question type in the fairytaleQA dataset, ground-truth questions that only share the context is used as the history of questions in the training mQG. During inference, we recursively feed previously generated questions, with the same context and question type, as the history of questions and give question type as a prefix to mQG. For the decoding method we use beam search; to exclude pre-generated questions we return multiple sequences from the beam search.

\subsection{Model Architecture}

% As shown in Figure \ref{fig:mQG-gen}, the encoder first takes a question type, desired to generate, and context as input, and $[SEP]$ token is inserted between those two. Then decoder generates a question based on the given input sequence. For the next generation step, the previously generated question is recursively fed to the encoder concatenated after the same question type and context, and separated with $[SEP]$ token. The generating step continues until desired question number per context per question type is reached. This recursive generation process enables mQG to generate multiple questions referencing previously generated questions for diversity.

In Figure \ref{fig:mQG-gen}, the architecture of mQG is shown. The encoder takes as input a question type, which represents the type of question to be generated, and a context, which provides the necessary information for generating questions. These two inputs are concatenated, with a $[SEP]$ token inserted between them. This concatenated input sequence is then passed through the encoder. Moving to the decoder, it generates a question based on the information provided by the encoder. For the next step, the previously generated question is recursively fed back into the model. Specifically, the previous question is concatenated with the same question type and context, and separated by a $[SEP]$ token. This concatenated sequence is then used as input for the next generation step. This recursive generation step continues until the desired number of questions per context per question type is reached.

The use of this recursive generation process in mQG allows the model to generate multiple questions while taking into account previously generated questions. This approach enhances the diversity of the generated questions and enables the model to reference and build upon its own previous outputs. By leveraging this architecture, mQG demonstrates its capability to generate a variety of questions that are contextually relevant and coherent. The recursive generation process contributes to the model's ability to produce diverse and meaningful questions in a controlled manner.

\begin{figure*}[ht]
\centerline
{\includegraphics[height=6.5cm]{images/mQG4.jpg}}
\caption{Overview of training process of mQG. $Question_1$ to $Question_m$ refer to ground-truth questions from the same context, without ground-truth question input to BART Decoder. The left table shows an example from the FairytaleQA dataset.}
\label{fig:mQG}
\end{figure*}

\subsection{Diversity Enhanced Training}
 \label{sec:qcl}

% \citet{su2022a} emphasized the importance of contrastive learning to encourage language models to generate diverse text. With contrastive learning, language models are able to make discriminative and isotropic token representations. We hypothesized that contrastive training can help mQG generate diverse questions. We introduce a novel question-aware contrastive objective $\mathcal{L}_{QCL}$ that reduces the similarity between a generated question and other questions from the same context. Given a sequence of output representation, which is output from decoder, $x = \{{x_1, ..., x_n}\}$ and sentence-level representation of ground-truth questions that are from the same context, $q = \{{q_1, ..., q_m}\}$. We concatenate two representations to $y = \{{y_1, ..., y_{(n+m)}}\}$, the $\mathcal{L}_{MQS}$ is calculated as
mQG is built upon the BART\citep{lewis-etal-2020-bart}, which has demonstrated remarkable performance in various natural language processing tasks. The primary pre-training objective of BART is to reconstruct the masked input based on unmasked input. To further leverage the capabilities of the pre-trained BART, we introduce a maximum question similarity loss. This loss is designed to promote similar representations for questions from the encoder and decoder. 

In Figure \ref{fig:mQG}, we give ground truth questions from the same context to the encoder as reference questions. The encoder processes the reference questions and produces their corresponding representations. Simultaneously, the decoder generates the representation for the targeted question. Following work by \citet{reimers-gurevych-2019-sentence}, we utilize mean pooling layers to convert question representations into sentence-level representations. The maximum question similarity loss is employed at this stage to encourage the sentence-level representations of the reference questions and the targeted question to become similar. 

Given a set of reference question sentence-level representations as $Q = \{{Q_1, ..., Q_m}\}$ and the sentence-level representation of the target question as $X$, the maximum question similarity 
loss ($\mathcal{L}_{MQS}$) is computed as follows:

\begin{equation}
\begin{aligned}
\mathcal{L}_{MQS} = & \frac{1}{m} \times \sum_{i=1}^{{m}} \max(0, s(Q_i,X))
\end{aligned}
\end{equation}
where $s(h_{y_i},h_{y_j})$ is a cosine similarity calculation between representations. By optimizing the model parameters to maximize the similarity between these representations, we ensure that mQG generates diverse questions. The overall training objective $\mathcal{L}$ is defined as 
\begin{equation}
\begin{aligned}
\mathcal{L} = \mathcal{L}_{CE} + \mathcal{L}_{MQS} 
\end{aligned}
\end{equation}
$\mathcal{L}_{CE}$ refers to the cross-entropy loss from a target question.
